"Well, Keep Thinking": Enhancing LLM Reasoning with Adaptive Injection Decoding

Large language models (LLMs) exhibit strong reasoning abilities, often attributed to few-shot or zero-shot chain-of-thought (CoT) prompting. While effective, these methods require labor-intensive prompt engineering, raising the question of whether reasoning can be induced without reliance on explicit prompts. In this work, we unlock the reasoning capabilities of LLMs without explicit prompting. Inspired by zero-shot CoT and CoT-decoding, we propose a novel decoding strategy that systematically nudges LLMs to continue reasoning, thereby preventing immature reasoning processes. Specifically, we monitor the model's generation and inject a designated phrase whenever it is likely to conclude its response prematurely, before completing the reasoning process. Our experimental evaluations on diverse reasoning benchmarks demonstrate that our proposed strategy substantially improves LLM reasoning capabilities, highlighting the potential of decoding-based interventions as an alternative to traditional prompting techniques.

==> tables/all_table_contents.tex <==
% 기본적으로 \tableCaption과 \tableContent을 정의 (초기 선언)
\providecommand{\tableCaption}{Llama3 8B / GSM8k - LLaMA outputs <eos> in 58.05\% of GSM8k problems.
}
\providecommand{\tableContent}{
        \textbf{Q:} Janet’s ducks lay 16 eggs per day. She eats three for breakfast every morning and bakes muffins for her friends every day with four. She sells the remainder at the farmers' market daily for 2 per fresh duck egg. How much in dollars does she make every day at the farmers' market? & \\
        \noalign{\vskip 0.2cm}
        \textbf{A:} <eos> &
    }


\ifcase \tableSelection
    % 0일 경우 아무 내용도 출력 안 함 (에러 방지)
\or
    % Case 1: silence (설명 + 내용)
\providecommand{\tableCaption}{
  Llama3 8B / GSM8k - LLaMA outputs <eos> in 58.05\% of GSM8k problems.
}

\providecommand{\tableContent}{
  \textbf{Q:} Janet’s ducks lay 16 eggs per day. She eats three for breakfast every morning and bakes muffins for her friends every day with four. 
  She sells the remainder at the farmers' market daily for \$2 per fresh duck egg. 
  How much in dollars does she make every day at the farmers' market? & \\[0.2cm]
  \textbf{A:} <eos> & 
}

% \renewcommand{\tableCaption}{Llama3 8B / GSM8k - LLaMA outputs <eos> in 58.05% of GSM8k problems.
% s}
%     \renewcommand{\tableContent}{
%         \textbf{Q:} Janet’s ducks lay 16 eggs per day. She eats three for breakfast every morning and bakes muffins for her friends every day with four. She sells the remainder at the farmers' market daily for $2 per fresh duck egg. How much in dollars does she make every day at the farmers' market? & \\
%         \noalign{\vskip 0.2cm}
%         \textbf{A:} <eos> &
%     }

\or
    % Case 2: 두 번째 테이블 (설명 + 내용)
\renewcommand{\tableCaption}{Gemma 7B / MultiArith - Repeats the given question instead of solving it.
}
    \renewcommand{\tableContent}{
        \textbf{Q:} The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? & \\
        \noalign{\vskip 0.2cm}
        \textbf{A:} The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\  \\ The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples &
    }
\or
    % Case 3: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Mistral 7B / CommonsenseQA - 42.49\% of Mistral's answers in CommonsenseQA generate unrelated grammar questions.}
        \renewcommand{\tableContent}{
            \textbf{Q:} What do people aim to do at work?
    (A) complete job
    (B) learn from each other
    (C) kill animals
    (D) wear hats
    (E) talk to each other
     & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} Random Topics: \\ Adjectives and AdverbsAdjectives and AdverbsAdjectives and Adverbs \\  \\ Next quiz: Grammar \\  \\ The ________ of the sentence is the subject. \\  \\ A. verb \\ B. noun \\ C. adjective \\ D. adverb \\ ============================ &
        }
\or
    % Case 4: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Mistral 7B / MultiArith - Outputs irrelevant numeric sequences while solving problems.}
        \renewcommand{\tableContent}{
            \textbf{Q:} Ned had to wash 9 short sleeve shirts and 21 long sleeve shirts before school. If he had only washed 29 of them by the time school started, how many did he not wash? & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} 1. 2. 3. 4. 5. 6. 7. 8. 9. 10. 11. 12. 13. 14. 15. 16. 17. 18. 19. 20. 21. 22. 23. 24. 25. 26. 27. 28. 29. 30. 31. 32. 33. 34. 35. 36. 37. 38. 39. 40. 41. 42. 43. 44. 45. 46. 47. 48. 49. 50. 51. 52. 53. 54. 55. 56. 57. 58. 59. 60. 61. 62. 63. 64. 65. 66. 67. 68. 69. 70. 71. 72. 73. 74. 75. 76. 77. 78. 79. 80. 81. 82. 83. 84. 85. 86. 87. 88. 89. 90. 91. 92. 93. 94. 95. 96. 97. 98. 99. 100. 101. 102. 103. 104. 105. 106. 107. 108. 109. 110. 111. 112. 113. 114. 115. 116. 117. 118. 119. 120. 121. 12 &
        }

\or
    % Case 6: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Llama3 8B / CommonsenseQA - Produces additional, unnecessary choices in multiple-choice scenarios.}
        \renewcommand{\tableContent}{
            \textbf{Q:} When drinking booze what can you do to stay busy?
    (A) reach tentative agreement
    (B) stay in bed
    (C) stop bicycle
    (D) examine thing
    (E) suicide & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} (F) stay busy \\ (G) stay sober \\ (H) stay in shape \\ Answer: F \\ Explanation:   When drinking booze what can you do to stay busy? \\ When drinking booze what can you do to stay busy? &
        }

\or
    % Case : 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Gemma 7B / logical deduction - Provides an answer first before reasoning through it.
}
        \renewcommand{\tableContent}{
            \textbf{Q:} The following paragraphs each describe a set of five objects arranged in a fixed order. The statements are logically consistent within each paragraph. On a shelf, there are five books: a brown book, a yellow book, an orange book, a green book, and a gray book. The green book is to the left of the gray book. The brown book is the third from the left. The gray book is the second from the right. The yellow book is to the left of the green book.\\ 
            Options:\\
                (A) The brown book is the third from the left\\ 
                (B) The yellow book is the third from the left\\
                (C) The orange book is the third from the left\\ 
                (D) The green book is the third from the left\\ 
                (E) The gray book is the third from the left & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} (C) The orange book is the third from the left\\ \\ 
                    Solution: \\ \\ 
                    The green book is to the left of the gray book.\\ 
                    The brown book is the third from the left.\\ 
                    The gray book is the second from the right.\\ 
                    The yellow book is to the left of the green book.\\ \\ 
                    The green book is to the left of the gray book.\\ 
                    The brown book is the third from the left.\\ 
                    The gray book is the second from the right.\\ 
                    The yellow book is to the left of the green book.\\ \\ 
                    The green book is to the left of the gray book.\\ 
                    The brown book is the third from the left.\\ 
                    The gray book is the second from the right.\\ 
                    The yellow book is to the left of the green book.\\ \\ 
                    The green book is to the left of the gray book.\\ 
                    The brown book is the third from the left.\\ 
                    The gray book is the second from the right.\\ 
                    The yellow book is to the left of the green book.
                     &
        }


\or
    % Case 7: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Gemma 7B / MultiArith - Arbitrarily generates answer choices even for non-multiple-choice questions.}
        \renewcommand{\tableContent}{
            \textbf{Q:} Luke was helping the cafeteria workers pick up lunch trays, but he could only carry 4 trays at a time. If he had to pick up 20 trays from one table and 16 trays from another, how many trips will he make? & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} A. 4 \\  \\ B. 5 \\  \\ C. 6 \\  \\ D. 7 \\  \\ E. 8 \\  \\ Show more \\ Step 1 \\ 1 of 2 \\  \\ Determine the number of trips Luke will make. \\  \\ $\begin{gather*} 20 \div 4 = 5 \text{ trips} \end{gather*} $ \\  \\ Result \\ 2 of 2 \\  \\ B. 5 &
        }

\or
% Case 8: 세 번째 테이블 (설명 + 내용)
\renewcommand{\tableCaption}{%
  Mistral 7B / multiArith - Frequently observed in Mistral:
  generates \# Guidance, \#Example in few-shot style,
  and solves in \#Guided Practice Revisited format.
}

\renewcommand{\tableContent}{%
\textbf{Q:} The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? & \\
\noalign{\vskip 0.2cm}
\textbf{A:} 26 \\[6pt]
\#\#\# Guidance \\[6pt]
The distributive property is a property of multiplication that allows us to distribute a factor over a sum or difference. \\[6pt]
\[
\begin{aligned}
3(a+b) &= 3a + 3b \\
5(a-b) &= 5a - 5b
\end{aligned}
\]
\\[6pt]
The distributive property is used to simplify expressions. \\[6pt]

\#\#\#\# Example A \\[4pt]
Simplify: \$5(a+b)\$ \\[4pt]
Solution: Use the distributive property to distribute the 5 over the sum. \\[4pt]
\[
\begin{aligned}
5(a+b) &= 5a + 5b \\
       &= 5a + 5b
\end{aligned}
\]
\\[6pt]

\#\#\#\# Example B \\[4pt]
Simplify: \$3(a-b)\$ \\[4pt]
Solution: Use the distributive property to distribute the 3 over the difference. \\[4pt]
\[
\begin{aligned}
3(a-b) &= 3a - 3b \\
       &= 3a - 3b
\end{aligned}
\]
\\[6pt]

\#\#\#\# Example C \\[4pt]
Simplify: \$2(a+b+c)\$ \\[4pt]
Solution: Use the distributive property to distribute the 2 over the sum. \\[4pt]
\[
\begin{aligned}
2(a+b+c) &= 2a + 2b + 2c \\
         &= 2a + 2b + 2c
\end{aligned}
\]
\\[6pt]

\#\#\#\# Concept Problem Revisited \\[4pt]
The school cafeteria had 23 apples. If they used 20 to make lunch for the students and then bought 6 more, how many apples would they have? \\[6pt]
The cafeteria had 23 apples. They used 20 to make lunch for the students. They bought 6 more. \\[4pt]
\[
\begin{aligned}
23-20 &= 3 \\
20+3  &= 23
\end{aligned}
\]
\\[6pt]

The cafeteria had 23 apples. They used 20 to make lunch for the students. They bought 6 more. \\[4pt]
\[
\begin{aligned}
23-20 &= 3 \\
20+3  &= 23
\end{aligned}
\]
\\[6pt]

The cafeteria had 23 apples. They used 20 to make lunch for the students. They bought 6 more. \\[4pt]
\[
\begin{aligned}
23-20 &= 3 \\
20+3  &= 23
\end{aligned}
\]
\\[6pt]

The cafeteria had 23 &
}


\or
    % Case 9: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Llama3 8B / MultiArith - Fails to derive the final answer by stopping CoT early despite having necessary components.}
    \renewcommand{\tableContent}{
        \textbf{Q:} Zoe was unboxing some of her old winter clothes. She found 8 boxes of clothing and inside each box there were 4 scarves and 6 mittens. How many pieces of winter clothing did Zoe have total? & \\
        \noalign{\vskip 0.2cm}
        \textbf{A:} 1. 8 scarves and 6 mittens 2. 8 scarves and 24 mittens 3. 32 scarves and 24 mittens 4. 32 scarves and 48 mittens \\ Zoe was unboxing some of her old winter clothes. She found 8 boxes of clothing and inside each box there were 4 scarves and 6 mittens. How many pieces of winter clothing did Zoe have total? 1. 8 scarves and 6 mittens 2. 8 scarves and 24 mittens 3. 32 scarves and 24 mittens 4. 32 scarves and 48 mittens &
    }

\or
    % Case 10: 세 번째 테이블 (설명 + 내용)
    \renewcommand{\tableCaption}{Mistral 7B / MultiArith - Creates and solves its own example instead of solving the given problem (forgetting issue).}
        \renewcommand{\tableContent}{
            \textbf{Q:} Paige had 43 math problems and 12 science problems for homework. If she finished 44 of the problems at school, how many problems did she have to do for homework? & \\
            \noalign{\vskip 0.2cm}
            \textbf{A:} "1. 43 2. 44 3. 45 4. 46 \\  \\ \#\#\# Watch This \\  \\ Watch this video for help with the concepts in this section. \\  \\ \#\#\# Guidance \\  \\ In the last section, we learned how to solve equations with fractions. In this section, we will learn how to solve equations with decimals. \\  \\ \#\#\#\# Example A \\  \\ Solve the equation for $x$ . \\  \\ $0.2x+0.3=0.5$ \\  \\ Solution: \\  \\ We can solve this equation by subtracting 0.3 from both sides. \\  \\ $0.2x+0.3-0.3=0.5-0.3$ \\  \\ $0.2x=0.2$ \\  \\ Now we can divide both sides by 0.2. \\  \\ $\frac{0.2x}{0.2}=\frac{0.2}{0.2}$ \\  \\ $x=1$ \\  \\ \#\#\#\# Example B \\  \\ Solve the equation for $x$ . \\  \\ $0.05x+0.02=0.07$ \\  \\ Solution: \\  \\ We can solve this equation by subtracting 0.02 from both sides. \\  \\ $0.05x+0.02-0.02=0.07-0.02$ \\  \\ $0.05x=0.05$ \\  \\ Now we can divide both sides by 0.05. \\  \\ $\frac{0.05x}{0.05}=\frac{0.05}{0.05}$ \\  \\ $x=1$ \\  \\ \#\#\#\# Example C \\  \\ Solve the equation for $x$ . \\  \\ $0.005x+0.002=0.007$ \\  \\ Solution: \\  \\ We can solve this equation by subtracting 0.002 from both sides. \\  \\ $0.005x+0.002-0.002=0.007-0.002$ \\  \\ $0.005x=0.005$ \\  \\ Now we can divide both sides by 0.005 \\ ============================" &
        }

\fi


==> tables/silence_template.tex <==
% \input{tables/all_table_contents} % 테이블 설명, 내용 불러오기

% \begin{table}[htbp]
% \centering
% \caption{\tableCaption}
% \label{tab:silence}

% \begin{tcolorbox}[
%   width=\textwidth,
%   colback=white,
%   colframe=black,
%   boxsep=5pt,
%   arc=2pt,
%   breakable
% ]
% \footnotesize
% % tabularx에서 폭 자동 조절: l열 + X열 (왼쪽, 오른쪽)
% \begin{tabularx}{\textwidth}{@{} l X @{}}
% \toprule
%   % 표 내용은 \tableContent에서 가져옴
%   % \tableContent 안에서 \noalign{\vskip ...}을 쓰지 말고,
%   % 필요한 경우 아래처럼 직접 줄바꿈 (\\[0.2cm]) 처리
%   \tableContent \\  % 마지막에 \bottomrule 앞에 행 하나를 맞추기 위해 \\ 추가
% \bottomrule
% \end{tabularx}

% \end{tcolorbox}
% \end{table}

